Evaluating the Robustness of Semantic Segmentation for Autonomous Driving against Real-World Adversarial Patch Attacks

Deep learning and convolutional neural networks allow achieving impressive performance in computer vision tasks, such as object detection and semantic segmentation (SS). However, recent studies have shown evident weaknesses of such models against adversarial perturbations. In a real-world scenario instead, like autonomous driving, more attention should be devoted to real-world adversarial examples (RWAEs), which are physical objects (e.g., billboards and printable patches) optimized to be adversarial to the entire perception pipeline. This paper presents an in-depth evaluation of the robustness of popular SS models by testing the effects of both digital and real-world adversarial patches. These patches are crafted with powerful attacks enriched with a novel loss function. Firstly, an investigation on the Cityscapes dataset is conducted by extending the Expectation Over Transformation (EOT) paradigm to cope with SS. Then, a novel attack optimization, called scene-specific attack, is proposed. Such an attack leverages the CARLA driving simulator to improve the transferability of the proposed EOT-based attack to a real 3D environment. Finally, a printed physical billboard containing an adversarial patch was tested in an outdoor driving scenario to assess the feasibility of the studied attacks in the real world. Exhaustive experiments revealed that the proposed attack formulations outperform previous work to craft both digital and real-world adversarial patches for SS. At the same time, the experimental results showed how these attacks are notably less effective in the real world, hence questioning the practical relevance of adversarial attacks to SS models for autonomous/assisted driving.

==> arxiv - Copia/attack_approach.tex <==
\section{Attack Formulation} \label{s:method}

This section presents the design of adversarial patches for semantic segmentation (SS), starting with a short recap of the basic notions behind SS. The patch optimization scheme for both the EOT-based and the scene-specific attacks is then presented. Finally, the proposed loss function is introduced.

%First, necessary background concepts of SS are recalled, then, the proposed patch optimization scheme is presented for both attacks, and, finally, the proposed loss function is introduced.


\subsection{Background on SS}
%An image with height $H$ and width $W$ can be represented as $x \in [0,1]^{N_p \times C}$, where $N_p = H \times W$ is the total number of pixels and $C$ is the number of channels.
An image with height $H$ and width $W$ can be represented as $x \in [0,1]^{H \times W \times C}$, %where $\matchcal{N_p}$ is the set of image pixels indexed as $\{1,2,..., H \times W\}$, and $C$ is the number of channels.
where $C$ is the number of channels.
An SS model returns $f(x) \in [0,1]^{H \times W  \times N_c}$, where $N_c$ is the number of classes.
This output represents the predicted class-probability scores associated to each image pixel.
In particular, $f_{i}^{j}(x) \in [0,1]$ denotes the predicted probability score for the $i$-th pixel of the image corresponding to the class $j$.
Consequently, the predicted semantic segmentation $SS(x) \in \mathbb{N}^{H \times W} $ is computed by extracting those classes with the highest probability score in each pixel: $SS(x) = { \argmax_{j \in \{1,...,N_c\} }}{f_i^j(x) } ~, \forall i \in \{1,...,H \times W\}$.

The ground truth for the SS of $x$ is defined as $y \in \mathbb{N}^{H \times W}$, and assigns the correct class (in $\{1,...,N_c\}$) to each pixel.
%The classic cross-entropy loss function $\mathcal{L}_{CE}(f_i(x), y_i) = -log({f_i^{y_i}(x)})$ is generally used to quantify the distance between the model prediction on each pixel $i$ and its ground truth class $y_i$. 
The performance of the SS models is evaluated by computing the cross-entropy loss $\mathcal{L}_{CE}(f_i(x), y_i) = -log({f_i^{y_i}(x)})$. Thus, for each pixel $i$, the model's prediction $f_i$ is compared against the ground truth class $y_i$.

\subsection{Patch-based attack pipeline}
%The general attack pipeline is the same for both attacks, and it is shown in Figure~\ref{fig:attack_scheme}. 
Both the EOT-based and the scene-specific attacks share a similar pipeline, which is explained in the following paragraph and illustrated in Figure~\ref{fig:attack_scheme}. 

\begin{figure}[!t]
\centering
\makebox[\columnwidth]{\includegraphics[scale=0.31]{img/attack_scheme.png}}
\caption{Outline of the proposed approach for crafting both the EOT-based and the scene-specific patches.}
\vspace{-1em}
\label{fig:attack_scheme}
\end{figure}


An adversarial patch of height $\tilde{H}$ and width $\tilde{W}$ is denoted as $\delta \in [0,1]^{\tilde{H} \times \tilde{W} \times C}$, where 
$\tilde{H}<H$ and $\tilde{W}<W$. This patch is then added to the original image $x$ to obtain a patched image $\tilde{x}$.
%, that is the actual input of the semantic segmentation model. 
Thus, the output of the SS model on this patched image would now be $f(\tilde{x})$.

The attacks considered are both untargeted. This means that the objective is to maximize a certain loss function $\mathcal{L}$, without forcing the classification of pixels towards any specific class.


%The objective of an adversarial patch is to mislead the model based on a certain loss function $\mathcal{L}$. %which depends on the model output.
%Since the paper focuses on untargeted attacks, the objective is to maximize the pixel-wise misclassification by the network, without forcing the classification of pixels towards any specific class.
%this is an untargeted attack, the objective is to maximize the error committed by the network, and, hence, the loss function.


% MOVE IN THE RELATED WORK
%The EOT method \cite{pmlr-v80-athalye18b} optimizes the adversarial patch across multiple images by applying transformations to help obtain an image-agnostic patch that is also more robust to the perturbations typical of a real world scenario (mainly changes in the point of view, camera noise, and changes in illumination).

Inspired by the EOT method \cite{pmlr-v80-athalye18b}, the idea is to find an optimal patch $\delta^*$ (starting from a random patch) that maximizes the loss $\mathcal{L}$ for all the patched images in expectation according to the distribution of transformations used to apply the patch $\delta$ on the image set $\mathbf{X}$.

Formally, we need to define:
%\begin{itemize}
\begin{compactitem}
%\begin{inparaenum}[(i)]
    \item A \textbf{set of appearance-changing transformations $\Gamma_a$}, for instance changes in illumination (brightness, contrast) and noise (uniform or gaussian). These transformations are directly applied to the patch, so obtaining a transformed patch $\zeta_a(\delta)$, where $\zeta_a\in\Gamma_a$. They are used to make the patch robust to illumination changes and acquisition noise. %The parameters for each of the transformations are randomized according to the range defined for the EoT;
    \item A \textbf{patch placement function $\eta$} that defines which portion of the original image $x$ is occupied by the patch. This is the only part of the pipeline that differs between the two proposed attacks, and is discussed further in the following subsections.
    \item A \textbf{patch application function $g(x,  \zeta_a(\delta), \eta)$} that replaces a certain area of $x$ with $\zeta_a(\delta)$ according to $\eta$ and returns the patched image $\tilde{x}$.
%\end{itemize}
\end{compactitem}
%\end{inparaenum}

These functions are sufficient to define both the \textit{EOT-based} attack, which uses randomized spatial transformations to place the patch onto the image, and the \textit{scene-specific} attack, which uses a precise projective transformation to enhance the accuracy of the patch placement.

\subsection{EOT-based patch attack}
The classic EOT-based attack, as in previous work \cite{brown_adversarial_2018}~\cite{2019arXiv191011099X}, 
uses a set of combinations of spatial transformations $\Gamma$, including translation and scaling, from which the patch placement function $\eta$ is selected.
%defines the patch placement function $\eta$ as an element of a set . 

The parameters for each transformation are randomized within a pre-defined range. Section~\ref{s:exp} provides a more detailed explanation of the set of transformations used.
The optimal patch is then defined as
%\useshortskip
\begin{equation}
    \delta^* = \argmax_{\delta} ~ \mathbb{E}_{x \in \mathbf{X}, \zeta_a \in \mathbf{\Gamma_a}, \eta \in \mathbf{\Gamma}} ~ 
    \mathcal{L}(f(\tilde{x}), y) ~
\end{equation}

% formula with sum
%\begin{equation}
%    \delta^* = \argmax_{\delta}\sum_{x \in \mathbf{X}} \sum_{\zeta \in \mathbf%{\Gamma}} {L_{CE}(f_i(\tilde{x}), y_i)}
%\end{equation}

% formula with expectation

%In practice, the optimal patch is computed with an iterative optimization process that modifies the pixels values at each step in the direction of the loss function gradient computed with respect to the patch at iteration $t$.
In practice, the optimal patch is computed via an iterative optimization process.
At each iteration $t$, the pixels values of the patch are modified in the direction of the gradient of the loss function computed with respect to the patch:
\useshortskip
\begin{equation}
    \delta_{t+1} = \mathrm{clip}_{[0,1]} \left(\delta_{t} + \epsilon \cdot\sum_{x \in \mathbf{X}} \sum_{\substack{\zeta_a\in\mathbf{\Gamma_a}\\ \eta\in \mathbf{\Gamma}}}\nabla_{\delta_{t}} \mathcal{L}(f(\tilde{x}), y) \right ),
\end{equation} \label{e:opt}
\noindent where $\epsilon$ represents the step size.
%Note that $\tilde{x} = g(x, \delta_t, \zeta)$  describes the patched image computed using the more recent patch $\delta_{t}$ and random transformations $\zeta \in \mathbf{\Gamma}$.
%$L$ consists of a weighted sum of multiple loss functions: an adversarial loss $L_{adv}$ (detailed in the following subsections), a smoothness loss $L_{S}$, and a non-printability score $L_{N}$. The first one is the core of the adversarial effect, while the others help improve the patch physical realizability, i.e., the transfer from a digital to a real-world scenario. Additional details about the other two losses are provided in the Appendix [REF]. 
$\mathcal{L}$ consists of a weighted sum of multiple loss functions. The adversarial patch effect is obtained through the optimization of the adversarial loss $\mathcal{L}_{adv}$ (discussed further in subsection \ref{subsection:loss}). Additionally, to ensure that the patch transfers well to the real world, two losses are added to account for the \emph{physical realizability} of the patch
%(see \cite{additional_material} for details)
(see supplementary material\footnote{The paper includes references to additional material, that can be provided upon request.}): smoothness loss $\mathcal{L}_S$ and non-printability score $\mathcal{L}_N$.
% WHEN REMOVING APPENDIX 

\subsection{Scene-specific patch attack} \label{subsection:scene-specific-approach}
To provide a more realistic approach for autonomous driving environments, this work proposes an alternative attack methodology that exploits the geometrical information provided by the CARLA Simulator~\cite{2017arXiv171103938D}. 

Here, the key assumption is the availability of an attackable 2D surface, e.g., a billboard, with a fixed location in close proximity to the road.
The CARLA simulator features the possibility to extract camera extrinsic and intrinsic matrices (details in supplementary material), and the pose of the attackable surface. The billboard-to-image transformations can be computed using a 3D roto-translation composition, which allows the patch to be warped accordingly, thus obtaining higher precision in applying the patch to the attack surface.
% WHEN REMOVING APPENDIX \cite{additional_material}

%This method allows the attacker to collect a dataset of several images $x \in \mathbf{X_\mathbf{s}}$ of the same scenario $\mathbf{s}$, together with the extrinsic and intrinsic matrices corresponding to each image that are used to compute the patch projective transformation. 


This attack uses the same optimization pipeline as before, with one major difference: instead of placing the patch randomly, as in the previous attack, correct projective transformations are used to determine the placement of the patch on the attackable surface. Hence, $\eta$ is no longer randomized, but is computed for each image in the dataset.


%This method allows a much more realistic patch placing and, hence, a simplified optimization process: EoT is not required anymore for the spatial placement of the patch since different viewpoints are taken into account intrinsically with the definition of a scene-specific dataset.
This method allows crafting precise attacks that are optimised for the region of the town that the attacker is interested in. The attacker would need to collect several images, from different viewpoints, of the desired attackable surface, along with the corresponding intrinsic and extrinsic matrices. This approach to image collection also implies that EOT is no longer needed for patch placement, thereby simplifying the optimization process.

The downside of this approach is that a digital representation of the target scene is required to accurately capture the required matrices. Although CARLA provides the possibility to import cities via OpenStreetMaps (\url{https://www.openstreetmap.org/}), it requires some amount of manual effort to properly model 3D meshes to include objects in this simulated world. These objects need to be properly designed to ensure that the patches optimised in simulation transfer well to the real-world.
%assets and meshes to be included in this simulated world. Also, to ensure that the optimized patches transfer well to the real-world from simulation, it would be pertinent to ensure that the assests be designed with semblance to reality.
%
Although this paper does not investigate CARLA-to-real-world transfer issues, future work will address this problem to improve the proposed methodology and adapt it for real-world attacks.
%
Section \ref{s:exp} provides a comparison of this method against the EOT-based attack.
%In the experimental parts \ref{s:exp}, multiple scene-specific attacks have been tested with different sizes of patches and sampled sequences. Additionally, a comparative evaluation is provided with the initial digital set of transformations, suggesting that a scene-specific adversarial patch is more robust and effective to attack a SS model in a autonomous driving scenario. 

%Regarding practical concepts, the previous approach has been developed thanks to the spatial points information available from the CARLA Simulator [CITE]. More details on the implementation part and computation of homogeneous matrices are provided in the Appendix [REF].


\subsection{Proposed loss function}\label{subsection:loss}
%To simplify the formalization, $\mathcal{N} = \{1,...,H \times W\}$ denotes the whole set of pixels in $\tilde{x}$ and $\mathcal{\tilde{N}} =\{1,..., \tilde{H} \times \tilde{W} \}  \subseteq \mathcal{N}$ only those that correspond to the patch $\delta$.

Cross-entropy (CE) is a popular choice as adversarial loss. Pixel-wise CE has been shown to work well when crafting an untargeted digital attack (i.e., by directly adding a perturbation $r$ to the pixels of a digital image)~\cite{nakka_indirect_2019}~\cite{bar_vulnerability_2021}.
This is formulated as: $\mathcal{L}_{adv}(f(x+r), y) = \frac{1}{|\mathcal{N}|}\cdot \sum_{i \in \mathcal{N}} \mathcal{L}_{CE}(f_i(x+r), y_i)$, where $\mathcal{N} = \{1,...,H \times W\}$ denotes the whole set of pixels in $\tilde{x}$.
However, modifications can be introduced to this formulation to allow crafting stronger attacks for fooling SS models.
%Previous works, such as  and \cite{bar_vulnerability_2021}, applied a pixel-wise cross-entropy loss function to optimize an untargeted digital perturbation $r$ for SS, i.e., $L_{adv}(f(x+r), y) = \frac{1}{N_p} \cdot \sum_{i=1}^{N_p} L_{CE}(f_i(x+r), y_i)$.
%Although a direct application of the cross-entropy loss function fits well to design adversarial patches for image classifiers (where only one probability score vector is provided as output), several improvements can be introduced to better fool an SS model. 


%In particular, given the prediction $SS(\tilde{x})$  of a patched image $\tilde{x}$, $\mathcal{N} = \{1,...,N_p\}$ denotes the whole set of image pixels and $\mathcal{\tilde{N}} =\{1,..., \tilde{N}_p \}  \subseteq \mathcal{N}$ those that are associated to the patch $\delta$.


Following previous notation, let $\mathcal{\tilde{N}} =\{1,..., \tilde{H} \times \tilde{W} \}  \subseteq \mathcal{N}$ denote only the pixels that correspond to the patch $\delta$. Then, $\mathbf{\Upsilon}$ defines a subset of image pixels that do not belong to the patch and are still predicted correctly by the model with respect to the trusted ground truth label $y$:
\useshortskip
\begin{equation}
\mathbf{\Upsilon} = \{ i \in  \mathcal{N} \setminus \mathcal{\tilde{N}} \quad | \quad SS_i(\tilde{x}) = y_i \}.
\end{equation}


Using $\mathbf{\Upsilon}$, the previous pixel-wise CE loss computed on $\mathcal{N} \setminus \mathcal{\tilde{N}}$ can be split into two distinct terms:
\useshortskip
\begin{equation}
    \mathcal{L}_M^{\tilde{x}}  =  \sum_{i \in \mathbf{\Upsilon}} \mathcal{L}_{CE}(f_i(\tilde{x}), y_i), \quad
    \mathcal{L}_{\overline{M}}^{\tilde{x}}  =  \sum_{i \notin \mathbf{\Upsilon}} \mathcal{L}_{CE}(f_i(\tilde{x}), y_i) ~.
\end{equation}

$\mathcal{L}^{\tilde{x}}_M$ describes the cumulative CE for those pixels that have been misclassified with respect to the ground truth $y$, while $\mathcal{L}^{\tilde{x}}_{\overline{M}}$ refers to all the others. 

Note that both $\mathcal{L}^{\tilde{x}}_M$ and $\mathcal{L}^{\tilde{x}}_{\overline{M}}$ do not consider pixels of the patch, which have been discarded to focus the optimization on attacking portions of the image away from the patch.
%The key idea is to exploit the previous two losses individually, avoiding that one obscure the gradient of the other. 
By computing these separate contribution to the total loss, we avoid that the contribution of the non-misclassified pixels gets obscured by the other term, which is a problem we found during preliminary tests.
Hence, the adversarial loss function gradient is redefined as follows:
\useshortskip
\begin{equation}
\nabla_{\delta} \mathcal{L}(f(\tilde{x}), y) = \gamma \cdot \frac{ \nabla_{\delta} \mathcal{L}_M^{\tilde{x}}}{||\nabla_{\delta} \mathcal{L}_M^{\tilde{x}}||_{2}} + (1-\gamma) \cdot \frac{ \nabla_{\delta} \mathcal{L}_{\overline{M}}^{\tilde{x}}}{||\nabla_{\delta} \mathcal{L}_{\overline{M}}^{\tilde{x}})||_{2}}  ~,
\end{equation}

%\noindent where $\gamma$ is a parameter that determines the importance of pixels not yet misclassified with respect to the adversarial stability of others. 
\noindent where $\gamma \in [0,1]$ is a parameter that determines whether the optimization should focus on decreasing the number of correctly classified pixels or improving the adversarial strength for the currently misclassified pixels.
The rationale of $\gamma$ is to provide an empirical balancing between the importance of $\mathcal{L}_M$ and $\mathcal{L}_{\overline{M}}$ at each iteration $t$ depending on the number of pixels not yet misclassified.
%Note that this loss function is a generalization of the standard cross-entropy, which can be obtained from this formulation by setting $\gamma = 0.5$. 



%The idea is to boost the number of misclassified points during the first part of the optimization process and then improve their strength as they increase.
Moreover, an adaptive value of $\gamma = \frac{|\Upsilon|}{|\mathcal{N} \setminus \mathcal{\tilde{N}}|}$ has been proposed to provide an automatic tuning of $\gamma$ at each iteration. 
The idea is to initially focus on boosting the number of misclassified points. 
Over time, as this number increases, the focus of the loss function gradually shifts toward improving the adversarial strength of the patch on these wrongly classified pixels.

%Section \ref{s:exp} provides an extensive analysis of $\gamma$  by comparing $\gamma = 0.5$ (i.e., standard pixel wise cross-entropy), $\gamma = 1.0$, and an the previous adaptive value, suggesting that this formulation is indeed more general and effective for SS models.

Section \ref{s:exp} provides an extensive analysis of the proposed loss function by comparing multiple values of $\gamma$ with the standard pixel wise CE measured both on $\mathcal{N} \setminus \mathcal{\tilde{N}}$ and $\mathcal{N}$ (which is used by \cite{nakka_indirect_2019}), suggesting that our formulation is indeed more general and effective for this kind of attack.

==> arxiv - Copia/conclusions.tex <==
\section{Conclusions and future work} \label{s:conclusions}

This paper presented an extensive study of the adversarial robustness of semantic segmentation models. This was accomplished by extensively evaluating the effect introduced by adversarial patches, to investigate the limits of real-world attacks for segmentation neural networks in an autonomous driving scenario.
Carrying out the investigations with increasingly ``real-world" benchmarks, we studied the effect of non-robust and EOT-based patches on the Cityscapes dataset, on a virtual 3D scenario, and in a real-world setting. We also introduced a new method called \textit{scene-specific attack}, which improves the EOT formulation for a more realistic and effective patch placement. 

The novel loss function introduced in the paper enabled to advance the state-of-the-art for adversarial patches optimization methods, as it proved to be a more general and efficient alternative to the classic cross-entropy function for this kind of problems.

This exhaustive set of experiments practically opens to a new point of view for studying SS models in autonomous driving. Although the proposed attacks were able to reduce the baseline model accuracy, the SS models proved to be somehow robust to real-world patch-based attacks. This was especially noticeable when the tests were performed in more realistic settings using CARLA and the real world, where, in most cases, the patch only affected the proximity of the attacked surface.

Nevertheless, this is a promising result, since it shows how the prediction provided by these models is not easily corruptible, especially in real-world scenarios. This is in contrast with previous work on patch-based adversarial attacks against classification and object detection models.

Future work will further investigate the robustness properties of these models, introducing defense mechanisms and trying to enhance the robustness of SS model by adding a temporal dimension. 
\vfill

==> arxiv - Copia/exp.tex <==
\section{Experimental results} \label{s:exp}
%{\color{blue}
This section describes the experimental setup and the results achieved with the proposed attacks. %\textit{EOT-based} and \textit{scene-specific} attacks.
%
%i.e. \textit{EOT-based} and \textit{scene-specific}, are presented.
%This section present the experimental results. First, the experimental setup is described, then the results for the two attacks are presented. 
%In particular, we first present the attack results obtained for the EOT-based attack without actually using EOT (hence yielding a "static digital patch attack, with fixed position and dimension) in order to provide an ablation study and to compare our results different loss functions involved in previous work. Then, the actual EOT-based attack is carried on the Cityscapes dataset.
%In particular, we first present the attack results obtained on the Cityscapes dataset with and without EOT. To provide an ablation study and to compare our results, different loss functions have been compared.
First, the proposed loss function is evaluated for different values of $\gamma$ comparing its effectiveness against the standard pixel-wise CE, showing that it is a better alternative for this kind of problems. Following this, the results of patches crafted with and without EOT are presented on the Cityscapes dataset. %This comparison shows how the generalized loss function can be combined with EOT, thereby presenting a set of transformations fit for the use case of autonomous driving.

%Then, results of the noEOT (i.e., without robust transformations) and EOT-based attack on the Cityscapes dataset are presented.
%}
%
Subsequently, the results obtained with the scene-specific attack on three CARLA-generated datasets are presented. These results are compared against the EOT-based attack to show the improved effectiveness of this formulation.
%
Finally, some preliminary results of real-world adversarial patches are presented.
%{\color{blue}
A more detailed analysis of all models tested against these attacks can be found in the supplementary material.%\cite{additional_material}.

%It is worth noting that additional supplementary experiments are presented in \cite{additional_material} to provide a fully robustness analysis of the tested models against these attacks.
%}

\subsection{Experimental setup} \label{s:exp_setup}
%All the experiments were performed on a set of GPUs, namely 8 NVIDIA-A100. The Carla simulator is running on [INSERT CARLA PC]. 
The experiments were performed on a set of 8 NVIDIA-A100 GPUs, while the CARLA simulator was run on a system powered by an Intel Core i7 with 12GB RAM and a GeForce GTX 1080 Ti GPU.

All experiments were performed in PyTorch~\cite{pytorch}. The optimizer of choice was Adam \cite{adam}, with learning rate set to 0.5 empirically. The effect of the adversarial patches on the SS models was evaluated using the mean Intersection-over-Union (mIoU) and mean Accuracy (mAcc) \cite{minaee_image_2020}.

%All the optimizations were performed using the PyTorch~\cite{pytorch} framework and the attacks were evaluated by measuring the mean-Intersection-over-Union (mIoU) and mean Accuracy (mAcc). These metrics are the most popular choice to evaluate the performance of an SS model on a given dataset \cite{minaee_image_2020}.The Adam optimizer \cite{adam} with a learning rate $0.5$ was utilised, keeping all other parameters unchanged. 

%All the following optimizations have been performed using the Adam optimizer \cite{adam} with a learning rate $0.5$. This parameter was decided based on the best results obtained among multiple experiments. The other Adam parameters are the original default values.
The repository link with the code used for all the experiments was not included for double-blind requirements, but it will be inserted upon request or acceptance.

\vspace{-1.2em}
\paragraph{Datasets}
The experiments in the case of driving images were carried out using the \textit{Cityscapes} dataset \cite{DBLP:conf/cvpr/CordtsORREBFRS16}, a popular benchmark for urban scene SS. The dataset consists of 2975 and 500 high resolution images ($1024\times2048$) for training and validation, respectively. The experiments reported in this paper were conducted on 250 images randomly sampled from the training set. Conversely, the entire validation set was used to evaluate the effectiveness of the patches.

\begin{comment}
To realize digital patches, we used the \textit{Cityscapes} dataset \cite{DBLP:conf/cvpr/CordtsORREBFRS16} that is one of the most popular benchmarks for SS. It consists of 500 and 2500 high resolution images ($1024\times2048$) for the validation and training set, respectively. The patches optimization is performed among 250 random images taken by the training set and then their effects are evaluated on the whole validation set. 
\end{comment}

% TODO discuss the three scenes and the effect of the real-world dimension of the patch/camera-billboard distance.
The CARLA simulator was used to provide a 3D virtual scenario. This set of experiments was performed in Town01, one of the built-in maps provided with the simulator, with `CloudyNoon' as the preset weather. To mimic the settings of the Cityscapes dataset, RGB images of size $1024\times2048$, along with their corresponding SS tags, were collected by placing a camera on-board the ego vehicle. 

The SS models trained on Cityscapes had to be fine-tuned to ensure good performance on CARLA images. 600 images for fine-tuning, 100 for validation, and 100 for testing were collected by spawning the ego vehicle at random positions in Town01. Additional details about the fine-tuning can be found in the supplementary material.%\cite{additional_material}.

To study the effectiveness of the patches in CARLA, the map of Town01 was manually edited to include three billboards. Thus, without-EOT, EOT-based, and the scene-specific attacks were carried out at three different locations within Town01. The datasets for the attacks were collected by spawning the ego vehicle at random locations within the proximity of each billboard to emulate varying viewpoints from which the patch might be captured in the real-world. For each of the three billboards, 150 training images, 100 validation, and 100 test images were gathered. Details about the position and orientation of the billboard and the camera were stored to compute the roto-translations used in the scene-specific attack.% (discussed in Section \ref{subsection:scene-specific-approach}).

Lastly, to study the effects of adversarial patches in the real world, an additional dataset of 1000 images, hereafter referred to as \textit{Patches-scapes}, was collected by mounting an action camera on the dashboard of a vehicle using a setup similar that of the Cityscapes dataset, and then driving the vehicle within the streets of our city.


\begin{comment}
For the scene specific part, we performed a fine tuning on a personal \textit{CARLA-dataset} that is composed by 600 training images and 100 validation, which are selected randomly by multiple runs. Then scene specific optimization has been performed on additional 5 scenarios (not considered in the train and validation set). Each scenario consists of multiple sampled points of view of a certain CARLA environment, with X1 and X2 images used for the patch optimization and evaluation, respectively. In addition to all the previous images, also the ground truth labels are provided and the extrinsic and intrinsic matrices that are necessary for the scene-specific attack. More detail about the environmental settings used on the CARLA Simulator are in Appendix X.
Finally, to evaluate our patches in a real world scenario, we provide \textit{Pisa-scapes} that is dataset of images collected by driving around Pisa with a go-pro on the dashboard of the car. 
\end{comment}

\vspace{-1.2em}
\paragraph{Models} 
The attacks studied in this paper were evaluated using DDRNet~\cite{ddrnet_paper}, BiSeNet~\cite{bisenet_paper}, and  ICNet~\cite{icnet_paper}, which represent the state-of-the-art in real-time SS, making them preferable for the use case of autonomous driving. Additionally, PSPNet~\cite{pspnet_paper} was included in the study for the EOT-based attack on the CityScapes dataset, but not for the scene-specific attack on CARLA, since we are interested in real-time performance.

% The two attacks studied in this paper were evaluated using DDRNet~\cite{ddrnet_paper}, BiSeNet~\cite{bisenet_paper}, ICNet~\cite{icnet_paper}, PSPNet~\cite{pspnet_paper}, PSANet~\cite{psanet_paper}. The first three listed here represent the state-of-the-art in real-time SS, which makes them preferable for the use case of autonomous vehicles. PSPNet and PSANet, though not real-time, were included to compare our attacks against the ones performed by Nakka et. al.~\cite{nakka_indirect_2019}.


% To ensure fair evaluation, all experiments were performed using the original Cityscapes dimensions of $1024\times2048$, without cropping. Thus, except PSANet, all other models were loaded with the pre-trained weights provided by the authors. The pre-trained model of PSANet, however, applied cropping to the images, and thus had to be trained from scratch. Further specifications of each of the models is provided in \ref{s:models}.



%{\color{blue}
%To ensure fair evaluation, all experiments were performed using the original Cityscapes dimensions of $1024\times2048$, without cropping. 
All the models were loaded with the pre-trained weights provided by the authors (further specifications are provided in the supplementary material.%\cite{additional_material}).
Table \ref{table:models_perf} summarizes the performance of these models on both the Cityscapes and CARLA validation sets. 
%}

%All the following tests consider available state of the art models for real-time and not real-time semantic segmentation: DDRNet~\cite{ddrnet_paper}, BiSeNet~\cite{bisenet_paper}, ICNet~\cite{icnet_paper}, PSPNet~\cite{pspnet_paper}, PSANet~\cite{psanet_paper}. The first three are famous real-time models that achieve more than 25 FPS, while the last two models are taken into consideration to provide a fair comparison with the work of Nakka et. al.~\cite{nakka_indirect_2019}. REF APP provides a comprehensive description of those models. 

%For Cityscapes, we used the original pretrained model (mentioned in REF APP) obtained with the original resolution $1024\times2048$. Subsequently, we performed a fine-tuning  among our Carla dataset for the scene-specific part. Table \ref{table:models_perf} summarized the performance of those models on both the Cityscapes and Carla validation sets. 


\begin{table}%[!t]
\centering
\resizebox{8.45cm}{!}{%
\begin{tabular}{|c|c|c|}
\hline
model        & \multicolumn{2}{c|}{mIoU / mAcc} \\ \hline
   & cityscapes      & CARLA (val - scene1 - scene2 -scene3)
\\ \hline
ICNet   & 0.78 ~/~0.85       & 0.70~/~0.84 - 0.53~/~0.70 - 0.64~/~0.74 - 0.62~/~0.74 \\ \hline
BiSeNet & 0.69~/~0.78       & 0.47~/~0.69 - 0.47~/~0.69 - 0.61~/~0.74 - 0.47~/~0.73      \\ \hline
DDRNet  & 0.78~/~0.85       & 0.72~/~0.88 - 0.54~/~0.74 - 0.62~/~0.76 - 0.64~/~0.78      \\ \hline
PSPNet  & 0.79~/~0.85       & nd      \\ \hline
%PSANet  & 0.00~/~0.00       & 0.00~/~0.00 - 0.00~/~0.00 - 0.00~/~0.00 - 0.00~/~0.00      \\ \hline
\end{tabular}
}

\caption{mIoU and mAcc of the tested models on Cityscapes (pre-trained) and our CARLA dataset (fine-tuned).}
\label{table:models_perf}
\vspace{-1em}
\end{table}



\subsection{EOT-based patches on Cityscapes}
%{\color{blue}
%This section illustrates the effectiveness of EOT for the use case of autonomous driving.
The Cityscapes dataset is used to optimize two types of patches on the same training images, one with EOT and the other without EOT (non-robust). Three different patch sizes are studied: $150\times300$, $200\times400$, and $300\times600$ pixels. 
%}

%This part illustrates the achieved results for digital adversarial attacks on the Cityscapes dataset with and without EOT. We optimized three different patch sizes: $150\times300$, $200\times400$, and $300\times600$ pixels. 

The non-robust patches (without EOT) were optimized by placing them at the center of the image at each training iteration (i.e., $\eta(\cdot) =$ fixed position) and applying no appearance transformations (i.e., $\Gamma_a =\emptyset$).

%As far as tests without EOT concern, the optimization is accomplished by placing the patch at the center of each optimized image (i.e., $\zeta(\cdot) =$ fixed position), and no appearance transformations were used (i.e., $\Gamma_a = \{\}$).

Conversely, the robust optimizations with EOT apply multiple digital transformations. $\Gamma_a$ includes only Gaussian noise with standard deviation 5\% of the image range.
$\Gamma$ includes random scaling ($80\% - 120\%$ of the initial patch size) and random translation defined as follows: if $(c_x, c_y)$ is the center of the image, the position of the patch is randomized within the range $(c_x\pm \tilde{r} \cdot \tilde{W}/2~,~c_y\pm \tilde{r} \cdot \tilde{H}/2)$, where $\tilde{r} \in [0,1]$ is a uniform random value.
The translation range was kept limited, rather than considering the full image space, to ensure a greater stability and faster convergence.
%and also a faster convergence of the optimization.
The patches were optimized over 200 epochs.
%All the following digital optimizations have been performed among 200 epochs. 


\vspace{-1.2em}
\paragraph{Loss functions analysis}
%{\color{blue}
Figure \ref{fig:digital_gamma_ablation} reports the mIoU obtained by training patches with the pixel-wise CE computed on $\mathcal{N}$ (used by \cite{nakka_indirect_2019}) and $\mathcal{N} \setminus \mathcal{\tilde{N}}$ compared to the extended CE loss proposed in this paper, with $\gamma \in \{ 0.5, 0.6, 0.7, 0.8, 0.95, 1.0, \frac{|\Upsilon|}{|\mathcal{N} \setminus \mathcal{\tilde{N}}|}\}$. Among the models evaluated in the paper, ICNet~\cite{icnet_paper} appears to be most robust on the Cityscapes dataset. Thus, the loss functions are studied by optimizing a $200\times400$ patch with and without EOT on ICNet.


%Figure \ref{fig:digital_gamma_ablation} reports an analysis of the validation set mIoU among optimizations epochs on the ICNet model~\cite{icnet_paper} (that appears to be the most robust model in all the performed tests), using a patch size equal to $200\times400$. It provides a comparison of multiple optimizations with and without EOT: the new proposed loss function formulation (with $\gamma = 0.5, 0.6, 0.7, 0.8, 0.95, 1.0, \frac{|\Upsilon|}{|\mathcal{N} \setminus \mathcal{\tilde{N}}|}$), and a pixel-wise CE computed on $\mathcal{N}$ (used by \cite{nakka_indirect_2019}) and $\mathcal{N} \setminus \mathcal{\tilde{N}}$.

For all the tested values of $\gamma$, our formulation converges to a higher attack effect (i.e., smaller mIoU) with lesser number of epochs than the one based on the pixel-wise CE. Experiments without EOT show that all the compared implementations converge after only $10$ epochs.
In the EOT case, the advantages are even more evident: our proposed formulation converges at almost 25 epochs, while the CE cases still reduce slowly at 200 epochs (nearly $6$ hours of optimization time).

The same study was performed for the scene-specific attack in the CARLA virtual world, and produced similar results, reported in the supplementary material.%\cite{additional_material}.

\vspace{-1.2em}
\paragraph{Adversarial patch effects.} %Table \ref{table:results_digital} reports all the achieved results. 
Table \ref{table:results_digital} reports how varying the patch size affects each of the SS models. We used the adaptive $\gamma$ (i.e., $\gamma=\frac{|\Upsilon|}{|\mathcal{N} \setminus \mathcal{\tilde{N}}|}$) that has shown the best overall effect among multiple experimental tests. 
%TODO NEXT
%(for sake of completeness, REF APP reports same tests with other values of $\gamma$ and CE).


Figure \ref{fig:digital_exps} illustrates the effects of the optimized patches on the BiSeNet model.
As expected, the non-robust patches (without EOT) obtain better attack performance with respect to the ones optimized with EOT. This is because the optimization process is simpler when not considering the randomized transformations. However, it is important to note that these patches would not be transferrable to the real world, and are not robust even to simple transformations \cite{2017arXiv171100117G, 2021arXiv210111466N}.

%TODO NEXT
%Moreover, we provide additional tests in REF APP to point out the weakness of those patches against simple digital translation. 
%}

 
\begin{figure*}[!t]
\centering
\makebox[\columnwidth]{\includegraphics[scale=0.38]{img/digital_gamma_ablation.png}}
\vspace{-1em}
\caption{Comparison of adversarial patch optimizations ($200 \times 400$) on ICNet and Cityscapes using different loss functions: two versions of the standard pixel-wise cross-entropy and our formulation with multiple values of $\gamma$. 
%The loss function used by %\cite{bar_vulnerability_2021, metzen_universal_2017, nakka_indirect_2019} 
%\cite{nakka_indirect_2019} 
%is the orange one ($\mathcal{L}_{CE}$ on $\mathcal{N}$), while the blue one is an our improved version that still %consider the common $\mathcal{L}_{CE}$.  
$\mathcal{L}_{CE}$ on $\mathcal{N}$ is the original version used by \cite{nakka_indirect_2019}, while $\mathcal{L}_{CE}$ on $\mathcal{N} \setminus \mathcal{\tilde{N}}$ is an improved version based on the rationale presented in Section \ref{s:method}.}
%}
\label{fig:digital_gamma_ablation}
\end{figure*}


\begin{table*}[!t]
\centering
\small
\begin{tabular}{|c|c|l|c|l|c|l|}
\hline
Model   & \multicolumn{6}{c|}{\begin{tabular}[c]{@{}c@{}}mIoU  |  mAcc \quad(rand / with EOT / without EOT)\end{tabular}}         \\ \hline
        & \multicolumn{2}{c|}{150x300}          & \multicolumn{2}{c|}{200x400}          & \multicolumn{2}{c|}{300x600}          \\ \hline
ICNet   & 0.70 / 0.58 / 0.54 & 0.81 / 0.69 / 0.65 & 0.67 / 0.50 / 0.45 & 0.79 / 0.61 / 0.55 & 0.60 / 0.38 / 0.28 & 0.72 / 0.42 / 0.34 \\ \hline
BiSeNet & 0.63 / 0.45 / 0.39 & 0.74 / 0.61 / 0.55 & 0.61 / 0.29 / 0.21 & 0.71 / 0.43 / 0.34 & 0.54 / 0.19 / 0.05 & 0.65 / 0.31 / 0.15 \\ \hline
DDRNet  & 0.73 / 0.65 /0.55 & 0.82 / 0.76 / 0.64 & 0.71 / 0.59 / 0.42 & 0.80 / 0.69 / 0.50 & 0.65 / 0.45 / 0.09 & 0.73 / 0.53 / 0.19 \\ \hline
PSPNet  & 0.76 / 0.42 / 0.33 & 0.82 / 0.57 / 0.45 & 0.73 / 0.23 / 0.00 & 0.79 / 0.30 / 0.05 & 0.67 / 0.01 / 0.00 & 0.73 / 0.06 / 0.05  \\ \hline
%PSANet  & nd / nd /nd & nd / nd /nd & nd / nd /nd & nd / nd /nd & nd / nd /nd & nd / nd /nd  \\ \hline
\end{tabular}
\caption{Adversarial patch results on the Cityscapes dataset. Each cell reports the final mIoU obtained with a random patch (no optimization), with EOT, and without EOT.}
\label{table:results_digital}
\end{table*}

\begin{figure*}[!t]
     \centering
     \begin{subfigure}{0.19\textwidth}
         \centering
         \includegraphics[width=\textwidth]{img/digital_results/imm_or.png}
         \vspace{-1.5em}
         \caption{}
         \label{fig:digital_exps_a}
     \end{subfigure}
     \begin{subfigure}{0.19\textwidth}
         \centering
         \includegraphics[width=\textwidth]{img/digital_results/original.png}
         \vspace{-1.5em}
         \caption{}
         \label{fig:digital_exps_b}
     \end{subfigure}
     \begin{subfigure}{0.19\textwidth}
         \centering
         \includegraphics[width=\textwidth]{img/digital_results/rand.png}
         \vspace{-1.5em}
         \caption{}
         \label{fig:digital_exps_c}
     \end{subfigure}
     \begin{subfigure}{0.19\textwidth}
         \centering
         \includegraphics[width=\textwidth]{img/digital_results/wEOT_patch.png}
         \vspace{-1.5em}
         \caption{}
         \label{fig:digital_exps_d}
     \end{subfigure}
     \begin{subfigure}{0.19\textwidth}
         \centering
         \includegraphics[width=\textwidth]{img/digital_results/woEOT_patch.png}
         \vspace{-1.5em}
         \caption{}
     \end{subfigure}
        \vspace{-1em}
        \caption{Semantic segmentations obtained from BiSeNet with no patch (b), a random patch (c), an EOT-based patch (d), and non-robust patch (without EOT) (e) added into a original image (a) of the Cityscapes validation set.}
        \vspace{-1em}
        \label{fig:digital_exps}
\end{figure*}

%\paragraph{Translation robustness analysis (Appendix?)}
%Point out how adversarial patches computed without EOT are not robust against translation. 

\subsection{Scene-specific patches on CARLA}
%The scene-specific attack is performed on the models defined earlier, that were fine-tuned on a training set of images generated with CARLA. 
The scene-specific attack was performed on the same set of models as defined earlier. Each of these models were first fine-tuned on images generated via CARLA. The performance of these fine-tuned models on the CARLA datasets is summarized in Table \ref{table:models_perf}. Please note that the mIoU score is computed as an average of the per-class IoU scores, which, for CARLA, might get to 0 for some classes due to the presence of a few pixels belonging to non-common objects. % (additional details in Appendix \ref{s:carla}).

%As explained in the previous section, 
As described in Section \ref{subsection:scene-specific-approach}, the patch is optimized to be adversarial for a specific urban scene by reprojecting it on the attackable 2D surface, which, in this work, is a billboard placed in three different spots in the Town01 map of CARLA. 
%{
%\textcolor{blue}{
This section reports the effect of the scene-specific attack compared against the non-robust (without-EOT) and the EOT-based attacks.
%}
%This section analyzes the effect of the real-world dimension of the patch and the effect of the number of pixels for a given dimension. Finally, the scene-specific attack is compared against the EOT-based attack {\color{blue}within the CARLA simulator}.
%\textcolor{blue}{
%For each experiment, the patch is optimized with the corresponding method on the dataset specific for each scene. 
The optimized patch is composed of $150\times300$ pixels, imposing a real-world dimension of $3.75m \times 7.5 m$. Additional experiments on the effect of the real-world dimension of the patch and the number of pixels used are presented in the supplementary material.% \cite{additional_material}.
%}
%\textcolor{blue}{
For all the following experiments, $\Gamma_a$ includes contrast and brightness changes (both 10\% of the image range), and Gaussian noise (standard deviation 10\% of the image range). 
%}
%}

%----------START REMOVED---------------%
\iffalse
\vspace{-1.2em}
\paragraph{Effect of real-world dimension of the patch}
For the digital EOT attack, the dimension of the patch within the image depends on the number of pixels (and, when used, on the scaling factor). For the scene-specific attack, the dimension of the patch within the image depends on both the real-world dimension of the patch (which, at most, is the dimension of the billboard), and the distance and orientation between the camera and the attackable surface. %Since the position of the billboard is considered fixed, as in real-world scenarios, and there is no control on the trajectory followed by the car (since they navigate within the limits of the road), the only controllable factor that changes the dimension of the patch within the image is the real-world dimension of the patch. 
Figure \ref{fig:carla_dim_ablation} reports the results of the attack
in terms of mIoU for different real-world patch dimensions and for the three different scenes. The number of pixels is fixed to 150x300.

It is clear that the larger the patch, the larger the effectiveness of the attack, independently of the scene considered. This is caused by the larger portion of the image that is occupied by the patch and it is an expected result.

\vspace{-1.2em}
\paragraph{Effect of number of pixels} 
To understand the effect of the number of pixels on the attack performance, the real-world patch dimension is kept fixed to the maximum allowed (i.e., the dimension of the billboard), and the number of pixels is varied, keeping the same height/width ratio of 1/2. The results are summarized in Figure \ref{fig:carla_pix_ablation} and show that the attack becomes less effective when the number of pixels is too small or too large. This can be explained by observing that, when the number of pixels is high, the real-world pixels may become smaller than the image pixel (due to projection rescaling), making the optimization process not effective. On the other hand, having a few big real-world pixels reduces the degrees of freedom of the attack method.

\begin{figure}[!t]
     \centering
     \begin{subfigure}{0.485\textwidth}
         \centering
         \includegraphics[width=\textwidth]{img/dim_carla_ablation.png}
         \vspace{-1.5em}
         \caption{}
         \label{fig:carla_dim_ablation}
     \end{subfigure}
     \begin{subfigure}{0.48\textwidth}
         \centering
         \includegraphics[width=\textwidth]{img/pix_carla_ablation.png}
         \vspace{-1.5em}
         \caption{}
        \label{fig:carla_pix_ablation}
     \end{subfigure}
\vspace{-1em}
\caption{Ablation study for the real-world dimension of the patch (a) and for the number of pixels used to design the patch (b).}
\vspace{-1em}
\end{figure}

%While the dimension of the patch influences heavily the attack performance, the number of pixels does not. One would expect that more pixels should lead to higher attack performance, but there are a few effects to be considered. (i) the scene-specific dataset includes also images where the billboard is far from the camera. The corresponding projected patch is rescaled accordingly, and, if composed of too many pixels, the resolution is heavily affected; (ii) the presence of a larger number of pixels slows the optimization process down. These two factors combined produce better results for an intermediate number of pixels. 

This result highlights another advantage of using the scene-specific attack: a smaller number of pixels is required during the optimization. This speeds the optimization up. % and improves the attack performance.
For a given scene (i.e., a given distance between the camera and the patch) the optimal real-world pixel size is the one that makes it equal to the size of the pixel in the image.

For the final experiments described in the next subsection we chose a resolution of $150\times 300$, which is an average value that yields good performance for the entire range of the scaling applied. %looks like a good tradeoff between attack performance and the possibility to place the patch on the billboard in the Unreal Editor without too much rescaling. This is required for a fair comparison against the EOT-based attack, as explained in the next section.
%----------End REMOVED---------------%
\fi

\begin{table*}[!t]
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{|c|c|l|c|l|c|l|}
\hline
Model   & \multicolumn{6}{c|}{\begin{tabular}[c]{@{}c@{}}mIoU  |  mAcc \quad(rand / without EOT / EOT / scene-specific)\end{tabular}}         \\ \hline
        & \multicolumn{2}{c|}{Scene1}          & \multicolumn{2}{c|}{Scene2}          & \multicolumn{2}{c|}{Scene3}          \\ \hline
ICNet   & 0.51 / 0.51 / 0.49 / 0.48 & 0.60 / 0.60 /0.56 / 0.54 & 0.64 / 0.64 / 0.61 / 0.61 & 0.74 / 0.74 / 0.73 / 0.73 & 0.63 / 0.63 / 0.59 / 0.59 & 0.76 / 0.76 / 0.73 / 0.74  \\ \hline
BiSeNet & 0.44 / 0.42 / 0.36 / 0.31 & 0.63 / 0.61 / 0.55 / 0.49 & 0.60 / 0.60 / 0.58 / 0.58 & 0.76 / 0.75 / 0.74 / 0.74 & 0.47 / 0.46 / 0.46 / 0.45 & 0.74 / 0.73 / 0.73 / 0.73 \\ \hline
DDRNet  & 0.51 / 0.50 / 0.46 / 0.46 & 0.70 / 0.69 / 0.69 / 0.69 & 0.62 / 0.62 / 0.52 / 0.49 & 0.76 / 0.75 / 0.71 / 0.66 & 0.65 / 0.65 / 0.58 / 0.59 & 0.78 / 0.78 / 0.76 / 0.76 \\ \hline
%PSPNet  & 0.40 / 0.31 /0.34 & 0.63 /0.61 / 0.64 & 0.57 / 0.55 /0.00 & 0.76 / 0.74 /0.00 & 0.41 / 0.41 /0.00 & 0.69 / 0.70 /0.00 \\ \hline
%PSANet  & 0.00 / 0.00 /0.00 & 0.00 / 0.00 /0.00 & 0.00 / 0.00 /0.00 & 0.00 / 0.00 /0.00 & 0.00 / 0.00 /0.00 & 0.00 / 0.00 /0.00 \\ \hline
\end{tabular}
}
\vspace{-0.5em}
\caption{Adversarial patch results on the three scene CARLA datasets. The Table reports the mIoU and mAcc obtained with random, non-robust (without EOT), EOT-based and scene-specific patches.}
\vspace{-0.5em}
\label{table:results_carla}
\end{table*}

\begin{comment}
\begin{figure*}[t]
     \centering
     \begin{subfigure}{0.16\textwidth}
         \centering
         \includegraphics[width=\textwidth]{img/carla_results/ddrnet_2_img.png}
         \vspace{-1.5em}
         \caption{}
         \label{fig:carla_exps_a}
     \end{subfigure}
     \begin{subfigure}{0.16\textwidth}
         \centering
         \includegraphics[width=\textwidth]{img/carla_results/ddrnet_4_img.png}
         \vspace{-1.5em}
         \caption{}
         \label{fig:carla_exps_b}
     \end{subfigure}
     \begin{subfigure}{0.16\textwidth}
         \centering
         \includegraphics[width=\textwidth]{img/carla_results/ddrnet_6_img.png}
         \vspace{-1.5em}
         \caption{}
         \label{fig:carla_exps_c}
     \end{subfigure}
     \begin{subfigure}{0.16\textwidth}
         \centering
         \includegraphics[width=\textwidth]{img/carla_results/ddrnet_2_pred.png}
         \vspace{-1.5em}
         \caption{}
         \label{fig:carla_exps_d}
     \end{subfigure}
     \begin{subfigure}{0.16\textwidth}
         \centering
         \includegraphics[width=\textwidth]{img/carla_results/ddrnet_4_pred.png}
         \vspace{-1.5em}
         \caption{}
     \end{subfigure}
     \begin{subfigure}{0.16\textwidth}
         \centering
         \includegraphics[width=\textwidth]{img/carla_results/ddrnet_6_pred.png}
         \vspace{-1.5em}
         \caption{}
     \end{subfigure}
        \vspace{-1em}
        \caption{Original images extracted from the test dataset from scene 1 (a), and the corresponding semantic segmentation prediction by DDRNet with a random patch (b), a no-robust patch (c), an EOT-based patch (d), and a scene-specific patch (e).}
        \label{fig:carla_exps}
        \vspace{-1em}
\end{figure*}
\end{comment}


\begin{figure*}[!t]
     \centering
     \begin{subfigure}{0.19\textwidth}
         \centering
         \includegraphics[width=\textwidth]{img/carla_results/carla_ddrnet_new_img_scene.png}
         \vspace{-1.5em}
         \caption{}
         \label{fig:digital_exps_a}
     \end{subfigure}
     \begin{subfigure}{0.19\textwidth}
         \centering
         \includegraphics[width=\textwidth]{img/carla_results/carla_ddrnet_preds_random.png}
         \vspace{-1.5em}
         \caption{}
         \label{fig:digital_exps_b}
     \end{subfigure}
     \begin{subfigure}{0.19\textwidth}
         \centering
         \includegraphics[width=\textwidth]{img/carla_results/carla_ddrnet_preds_noeot.png}
         \vspace{-1.5em}
         \caption{}
         \label{fig:digital_exps_c}
     \end{subfigure}
     \begin{subfigure}{0.19\textwidth}
         \centering
         \includegraphics[width=\textwidth]{img/carla_results/carla_ddrnet_preds_eot.png}
         \vspace{-1.5em}
         \caption{}
         \label{fig:digital_exps_d}
     \end{subfigure}
     \begin{subfigure}{0.19\textwidth}
         \centering
         \includegraphics[width=\textwidth]{img/carla_results/carla_ddrnet_preds_specific.png}
         \vspace{-1.5em}
         \caption{}
     \end{subfigure}
        \vspace{-1em}
        \caption{(a) is an image extracted from the scene-1 test dataset augmented with a scene-specific patch optimized on DDRNet, while (e) is its corresponding SS; (b), (c), and (d) are predictions obtained by augmenting the same test image with a random, non-robust and EOT-based patches, respectively.}
        %from scene 1 (a), and the corresponding semantic segmentation prediction by DDRNet with a random patch (b), a no-EOT patch (c), an EOT-based patch (d), and a scene-specific patch (e).}
        \label{fig:carla_exps}
        \vspace{-1em}
\end{figure*}
%\vspace{-1.2em}
%\paragraph{Comparison against EOT attack}
%The following experiments are performed to compare the scene-specific and the EOT-based attacks. For each experiment, the patch is optimized with the corresponding method on the dataset specific for each scene. 

Since the objective of this work is to craft RWAEs, the performance of the attacks is evaluated by measuring the mIoU and mAcc scores on additional scene-specific datasets. These additional datasets are produced by collecting the same images of the validation set of each scene-specific dataset, but with a single major modification: the billboard object is modified in the \textit{Unreal Editor} \cite{unrealengine} by applying the optimized patch as a \emph{decal} object, which is a way to stick an image on a surface in the virtual environment. This method should provide a simulated real-world application of the patches, since they are no more applied directly on the image, but the image itself includes the patched billboard. %To provide a fair comparison, all the experiments are performed with $\gamma=1$, learning rate 0.5, 500 epochs, for patches of $150\times 300$ pixels.

Table \ref{table:results_carla} summarizes the results obtained on these three additional scene-specific datasets, with a random patch, a non-robust patch, an EOT-based patch, and a scene-specific patch. Figure \ref{fig:carla_exps} shows a comparison of all the discussed attacks on DDRNet.

For almost all the combinations of scene and network, the scene-specific attack outperforms the EOT-based attack, confirming that the scene-specific attack, for this kind of problems, is a better alternative to the EOT formulation for the placement of the patch within the image. The only case where the the two attacks show comparable performance is for scene 3, where the billboard is almost perpendicular to the camera plane, allowing the EOT method to cover realistic patch placing functions. 

%{\color{blue}
%However, regardless of the kind of attacks, the networks used in this paper are quite robust to adversarial patches, since the performance is not completely ruined, especially for some particular classes (the road class above all). 
It is also worth noting that SS models are rather robust to adversarial patch attacks in general. Although it is possible to craft adversarial patches that cause a section of the image to be wrongly segmented, it tends to be more difficult than fooling models for tasks such as classification. 
%}
Additional details are reported in the supplementary material.%\cite{additional_material}.

\subsection{Real-world patches}
In order to prove that the proposed pipeline can be used for a real-world attack, we use the \textit{Patches-scapes} dataset (described in Section \ref{s:exp_setup}) to craft an adversarial real-world patch using the EOT-based patch attack. This section presents the results of an attack in Figure \ref{fig:realworld}. %{\color{blue}Although the optimized patch does not alter portions of the image far from its position, a significant area of the predicted SS is affected by patch features, while the random patch does not.} 
Although the presence of the optimized patch does alter a significant area of the predicted SS (while the random patch does not), portions of the image far from its position are not affected. Furthermore, the attack performance decreases as we move the patch away from the camera (details provided in the supplementary material.%\cite{additional_material}).
%{\color{red} Further tests, provided in the , show how the attack performance decreases as we move the patch away from the camera.} 
The patch is optimized for 200 epochs on the pre-trained version of ICnet (since it showed good performance on the Patches-scapes dataset) and printed as a $1m \times 2m$ poster.

\begin{figure}[!t]
     \centering
     \begin{subfigure}{0.23\textwidth}
         \centering
         \includegraphics[width=\textwidth]{img/final_rand_rw_2.png}
         \vspace{-1.5em}
         %\caption{}
         \label{fig:realworld_a}
     \end{subfigure} %\quad
     \begin{subfigure}{0.23\textwidth}
         \centering
         \includegraphics[width=\textwidth]{img/final_adv_rw_2.png}
         \vspace{-1.5em}
         %\caption{}
         \label{fig:realworld_b}
     \end{subfigure}
        %\vspace{-1em}
        \caption{Real-world predictions on ICNet obtained with a printed random patch (left) and an optimized patch (right).}
        \label{fig:realworld}
        \vspace{-1em}
\end{figure}

Testing adversarial patches for autonomous driving in the real world poses a series of difficulties that heavily limited the tests. First, it is not easy to find a urban corner with good prediction accuracy, and which is not crowded with moving vehicles (which might be dangerous). Second, the patch must be printed in the highest resolution possible on a large rigid surface, which might get expensive. Furthermore, since weather conditions are not controllable and change throughout the day, results can diverge from what is expected. 

The scene-specific attack, which requires additional geometric information, could not be implemented at the time of writing, but will be considered in future work.




==> arxiv - Copia/intro.tex <==
\vspace{-1.5em}
\section{Introduction}
\vspace{-0.5em}
The rise of deep learning unlocked unprecedented performance in several scientific areas \cite{dl_appl}. 
%One of the fields that benefited most from these developments is computer vision.
Convolutional neural networks \cite{krizhevsky_imagenet_2017} (CNNs) yielded super-human performance for many different computer vision tasks, such as image recognition \cite{2015arXiv151207108G}, object detection \cite{2015arXiv150601497R} \cite{2015arXiv150602640R}, %reinforcement-learning-based game playing \cite{mnih}, 
 and image segmentation \cite{minaee_image_2020}. Image segmentation, and semantic segmentation (SS) in particular, is used in autonomous driving perception pipelines \cite{siam2018comparative}, mainly for object detection \cite{minaee_image_2020}. %Image segmentation can be categorized as (i) semantic segmentation, (ii) instance segmentation, and (iii) panoptic segmentation. The focus of this paper is on CNNs for semantic segmentation, which includes the majority of segmentation models in the literature  

%Despite their high performance, CNN-based architectures have attracted massive attention in the computer vision community also due to their vulnerability to adversarial attacks \cite{silva_opportunities_2020}. 

Despite their high performance, CNNs are prone to adversarial attacks \cite{silva_opportunities_2020}. Most of the literature on adversarial attacks focuses on directly manipulating the pixels of the whole image, hence making the assumption that the attacker has control over the digital representation of the environment obtained by the on-board cameras. This kind of unsafe inputs are called \emph{digital} adversarial examples.

 Although such digital attacks do not transfer well into the real world, they continue to be used to evaluate the robustness of models in safety-critical systems \cite{survey_trust, 
bar_vulnerability_2021, 
metzen_universal_2017}.
%{\color{blue} Although these attacks are difficult in real-world scenarios, recent studies still focus on them for evaluating the model robustness on safety-critical systems [CITE].}
% \cite{DBLP:journals/corr/LuSFF17}. Furthermore, if one assumes that the attacker has the possibility to tamper the digital data produced by cameras, likely the attacker also disposes of the access to other parts of the system, making adversarial attacks to CNNs less relevant.
%Conversely, real-world adversarial examples (RWAEs) are physical world objects that can be placed in the field of view of a camera, making the captured image to result adversarial for the attacked neural network \cite{kurakin_adversarial_2017}. RWAEs pose a significantly more dangerous threat to safety-critical systems, since they can induce errors in neural networks without having access to the digital representation of the image.
\emph{Real-world} adversarial examples (RWAEs), on the other hand, are physical objects that can be placed in the field of view of a camera, such that the resulting image acts as an adversarial example for the neural network under attack \cite{kurakin_adversarial_2017}. Thus, RWAEs can induce errors in neural networks without requiring the attacker to access the digital representation of the image, thereby making them a more realistic and dangerous threat to safety-critical systems.

%As such, this latter kind of AEs represents a more dangerous threat to safety-critical systems, since they can induce errors in neural networks without requiring the attacker to have access to the digital representation of the image.

% {\color{blue}
% As such, this work pose attention on RWAEs of attacks as a more realistic and credible tool for evaluating the models robustness in an Autonomous Driving scenario. 
% Among the several types of RWAEs proposed in the literature \cite{sun_survey_2018}, this work aims at crafting powerful adversarial patches, which are more compliant with an autonomous car environment, since \cite{brown_adversarial_2018} they can be printed and attached to billboards, signs, or any other visible 2D surface. It extremely important to note that, to the best of our knowledge, this work represents the first exhaustive evaluation on the robustness of SS models against real-world adversarial patches for autonomous driving systems.
%(PUT THIS IN THE RELATED PART)
%Furthermore, in order to provide a fair comparison with adversarial attacks proposed on the literature we also evaluated our pipeline on universal digital adversarial patches. 
% }

\begin{figure}[!t]
     \centering
     \begin{subfigure}{0.155\textwidth}
         \centering
         \includegraphics[width=\textwidth]{img/intro_img/random_patch_new.png}
         \vspace{-1.5em}
         \caption{}
         \label{fig:carla_exps_a}
     \end{subfigure}
     \begin{subfigure}{0.155\textwidth}
         \centering
         \includegraphics[width=\textwidth]{img/intro_img/imm_or_new.png}
         \vspace{-1.5em}
         \caption{}
         \label{fig:carla_exps_b}
     \end{subfigure}
     \begin{subfigure}{0.155\textwidth}
         \centering
         \includegraphics[width=\textwidth]{img/intro_img/wEoT_patch_new.png}
         \vspace{-1.5em}
         \caption{}
         \label{fig:carla_exps_c}
     \end{subfigure}
     \begin{subfigure}{0.155\textwidth}
         \centering
         \includegraphics[width=\textwidth]{img/carla_results/intro_carla_1.png}
         \vspace{-1.5em}
         \caption{}
         \label{fig:carla_exps_d}
     \end{subfigure}
     \begin{subfigure}{0.155\textwidth}
         \centering
         \includegraphics[width=\textwidth]{img/carla_results/intro_carla_2.png}
         \vspace{-1.5em}
         \caption{}
     \end{subfigure}
     \begin{subfigure}{0.155\textwidth}
         \centering
             \includegraphics[width=\textwidth]{img/carla_results/intro_carla_3.png}
             \vspace{-1.5em}
         \caption{}
     \end{subfigure}
        \vspace{-1em}
        \caption{Proposed adversarial patches on Cityscapes \cite{DBLP:conf/cvpr/CordtsORREBFRS16} (b) and CARLA Simulator \cite{2017arXiv171103938D} (e); (c/f) show the corresponding SS predicted by BiSeNet \cite{bisenet_paper}; (a/d) show the corresponding predictions obtained using random patches instead of adversarial ones.}
        \vspace{-1em}
        \label{fig:intro_exps}
\end{figure}


\smallskip
\noindent
\textbf{This paper.}
This work focuses on RWAEs, as they represent a potential threat to tasks in autonomous driving today. Although the effects of RWAEs have been studied extensively in the literature for classification and object detection, those on SS remain relatively unexplored. However, SS is an integral part of autonomous driving pipelines~\cite{siam2018comparative}. Thus, this paper examines various state-of-the-art models for real-time SS aiming at benchmarking their robustness to RWAEs in autonomous driving scenarios.

Of the several types of RWAEs proposed in the literature \cite{sun_survey_2018}, the form of attack used in this paper is adversarial patches \cite{brown_adversarial_2018}. This is because attacks that perturb the whole image are not practically feasible in the real world. Conversely, such patches can be easily printed and attached to any visible 2D surface in the driving environment, such as billboards and road signs, thus making them a simple, yet effective attack strategy.

The paper starts by recognizing the shortcomings of the standard cross-entropy loss for optimizing adversarial patches for SS. Thus, an extension to the cross-entropy loss is proposed and integrated in all the performed attacks. This extension forces the optimization to focus on pixels that are not yet misclassified, thus obtaining patches that are more powerful compared to those generated with the standard cross-entropy-based setting~\cite{nakka_indirect_2019}.

Following this rationale, the robustness of real-time SS models to RWAEs attacks is benchmarked. 
The paper starts by first examining the \textbf{case of driving images}, crafting adversarial patches on the Cityscapes dataset \cite{DBLP:conf/cvpr/CordtsORREBFRS16}, a popular benchmark of high-resolution images of urban driving.
Robust real-world patches are crafted by following the Expectation Over Transformation (EOT) \cite{pmlr-v80-athalye18b} paradigm, which has been extended in this work to attack SS models. 
Furthermore, a comparison against non-robust patches (without EOT) is presented to question their effectiveness on driving scenes. 
%Furthermore, a comparison with no-robust patches is proposed to introduce a clear concern with the state-of-the-art evaluations.

Another set of experiments targeted a \textbf{virtual 3D scenario}, for which a stronger adversarial attack is presented and tested. The proposed \emph{scene-specific attack}, defined in Section \ref{subsection:scene-specific-approach}, is a more practical tool for crafting adversarial patches in a realistic autonomous driving scenario. It assumes that the attacker is interested in 
targeting an autonomous driving scene at a particular corner of a specific town, where information about the position of the attackable 2D surface (in our case, a billboard) is available. To satisfy such requirements we developed and tested this attack using the CARLA simulator, which provides all the needed geometric information. These experiments include a comparison with the EOT-based and non-robust patches, performed by importing them into the CARLA world and placing them on billboards to simulate a realistic study. 

Figure \ref{fig:intro_exps} provides some examples of the effect of our patches on Cityscapes and CARLA.

%Finally, the benchmarks were concluded focusing to a \textbf{real 3D scenario} by performing a set of experiments in the real world.
The last set of experiments were conducted on a \textbf{real-world driving scenario}, which required collecting a dataset within the city, optimizing a patch on it, physically printing said patch on a billboard, and finally evaluating SS models on images containing the printed patch.

To the best of our knowledge, this work represents the first exhaustive evaluation of the robustness of SS models against RWAEs for autonomous driving systems. The results of the experiments state important observations that should be taken into consideration while evaluating the trustworthiness of SS models in autonomous driving. First, they demonstrate that non-robust patches are not good candidates for assessing the practical robustness of an SS model to adversarial examples. Indeed, while they proved to be effective in attacking images related to driving scenes (from Cityscapes), they do not induce any real-world adversarial effect when crafted and tested in a virtual 3D world (based on CARLA). 
Conversely, robust patches, crafted with EOT or the proposed scene-specific approach, resulted to be less effective than non-robust ones on Cityscapes images, but were capable to accomplish the attack in both virtual 3D world and the real world.
Nevertheless, their effectiveness in the latter two cases still resulted to be quite limited, hence questioning the practical relevance of RWAEs.

%, showing that the tested SS models tend to be reasonably robust to RWAEs. %making them a strong candidate to consider for improving trustworthiness of the Deep Learning pipeline in safety-critical systems. 
%This also suggests that SS should be better leveraged within the Deep Learning pipeline to help improve trustworthiness of safety-critical systems. 

In summary, the paper makes the following contributions:
\begin{compactitem}
 \item It proposes an extension to the pixel-wise cross-entropy loss to enable crafting strong patches for the semantic segmentation setting.
  \item It proposes a novel technique for crafting adversarial patches for autonomous driving scenarios that utilize geometric information of the 3D world.
   %\item It presents a pipeline that enables quick, flexible, and seamless crafting and evaluation of adversarial patches on a range of datasets from Cityscapes to the simulator and even to the physical world. 
 \item It finally reports an extensive evaluation of RWAE-based attacks on a set of real-time semantic segmentation models using data from the Cityscapes dataset, CARLA, and the real world.
\end{compactitem}

The remainder of this paper is organized as follows: Section \ref{s:related} provides a brief overview of related work existing in the literature, Section \ref{s:method} formalizes the proposed loss function, pipeline, and attack strategy, Section \ref{s:exp} reports the experimental results, and Section \ref{s:conclusions} states the conclusions and proposes ideas for future work.




%---------------------------------------------------------------------------
% OLD VERSIONS
%---------------------------------------------------------------------------

\begin{comment}
%\subsection{This paper}
\smallskip
\noindent
\textbf{This paper.}
{\color{blue}
This paper focuses on RWAEs. Being a more realistic and credible threat to autonomous systems today, the paper evaluates the response of Semantic Segmentation models to such attacks.
%being a more realistic and credible tool for evaluating a SS model of autonomous cars system.
Among the several types of RWAEs proposed in the literature \cite{sun_survey_2018}, this work aims at crafting powerful adversarial patches \cite{brown_adversarial_2018}. Since adversarial patches can be easily printed and attached to any visible 2D surfaces such as billboards or road signs, they prove to be a simple, yet effective attack for autonomous driving scenarios.

%that are more compliant with an autonomous car environment, since \cite{brown_adversarial_2018} they can be printed and attached to billboards, signs, or any other visible 2D surface.
%This paper proposes a more effective attacks pipeline for evaluating a SS model placed inside the perception system of Autonomous cars. This is accomplished by leveraging common adversarial patches with a new crafting scheme that is more consistent with a real-world evaluation and enriched with a more performing loss function. Firstly, we extended the 

Gradient-based optimization along with a new crafting pipeline enabled the generation and evaluation of adversarial patches in real-world scenarios. The paper starts by first examining robust and no-robust (even if universal) adversarial patches on the Cityscapes dataset \cite{DBLP:conf/cvpr/CordtsORREBFRS16}, that provides a high resolutions images extracted by urban scene from an autonomous car.
On this dataset, robust real-world patches are crafted following the Expectation Over Transformation (EOT) \cite{pmlr-v80-athalye18b} paradigm (discussed in Section 2), that has been extended in this work for SS attacks. 
%The adversarial examples thus generated are robust to various transformations typically found in the real world, such as changes in lighting, viewing angle and so on. A comprehensive evaluation of such crafting techniques for the specific case of SS models is performed by comparing the metrics on non-EOT vs EOT-based patches.

%These patches are generated by enhancing well-known gradient-based optimization with a new crafting pipeline, which is more compatible with a real-world scenario. Firstly, we examine robust and universal adversarial patches on the Cityscapes dataset [CITE]. They are crafted using an extended version of the Expectation Over Transformation (EOT) formulation \cite{pmlr-v80-athalye18b} for SS,  to produce adversarial examples robust to a set of transformations typically found in the real world. 

%In particular, to give a comprehensive evaluation, we produce both no-robust (i.e., without EOT transformations, usually involved in literature) and EOT patches, denoting that real-world appearances constraints significantly reduce the adversarial effect on the model outcome. Consequently, 

Consequently, a stronger adversarial attack is introduced and tested. The proposed \empth{scene-specific attack}, defined in Section \ref{subsection:scene-specific-approach}, is a more realistic tool for crafting adversarial patches in a real 3D environment as a autonomous driving scenario.  It assumes that the attacker is interested in %attacking autonomous vehicles in 
targeting autonomous vehicles at a particular corner of a specific town, where information about the position of the attackable 2D surface (in our case, a billboard) is available. To satisfy such requirements we develop and test this attack using the CARLA simulator that provide all the geometric information of its virtual 3D environment. These experiments provide also a comparison with the EOT approach and no robust patches by importing all the crafted patches inside the CARLA world as billboard to simulate a realistic analysis. 
%The effectiveness of the scene-specific attack was studied using the CARLA simulator \cite{2017arXiv171103938D}. The simulator allowed to easily collect a dataset of images from a car-mounted dashcam along with the corresponding camera-to-billboard relative poses, thereby allowing the adversarial patches to be tested in a variety of autonomous driving scenarios. During training, the patch is optimized on these images by digitally projecting the patch according to the corresponding camera-to-billboard transformation. This formulation provides a more realistic alternative to the EOT paradigm. 
Figure \ref{fig:intro_exps} provides some examples of the effect of our patches on Cityscapes and CARLA.
%As such, part of the experiments presented in this paper uses the CARLA simulator \cite{2017arXiv171103938D} which allow to easily collect a dataset of car-mounted dashcam images, along with the corresponding camera-to-billboard relative poses, and test them on autonomous driving scenarios.
%The second, called \emph{scene-specific attack}, assumes that the attacker wants to attack an autonomous driving system in a particular urban scene, for which the position of the attackable 2D surface (in our case, a billboard) is known. The Carla simulator \cite{2017arXiv171103938D} is utilised to collect a dataset of car-mounted dashcam images, the camera-to-billboard relative pose, and the camera intrinsic matrix. 

%Finally, a conclusive set of experiments examine physical patches, that were printed and tested in an outdoor environment.

Finally, the paper concludes by performing a small set of experiments in the real world. This involved collecting a dataset within the city, optimizing a patch on it, printing said patch and evaluating SS models on images containing the printed patch. However, these experiments were limited owing to the cost (both time and resources) of performing them.

%The paper also discusses an extension to the classic cross-entropy loss, proposed to ensure that at 

Additionally, the paper presents an extension to the classical cross-entropy loss to help craft powerful adversarial examples for SS models. The proposed extension ensures that at each training iteration the patch builds up ``adversarial-ness'' towards pixels that have not yet been misclassified. This extended version of the loss is evaluated on Cityscapes and CARLA datasets and was found to generate patches with higher adversarial effect when compared to the classical setting.

%To improve the crafting process, this work presents an extension of the classical cross-entropy loss, which ensures that at each training iteration the patch builds up ``adversarial-ness'' towards pixels that have not yet been misclassified. This new loss is embedded in the crafting pipelines of both Cityscapes and Carla, showing that it outperforms related strategies, always producing a higher adversarial effect.

%Furthermore, to show the improvements of the proposed attacks scheme a comparison with previous utilized loss function is shown even for a no real-world application. 

The effectiveness of our adversarial formulations is evaluated via extensive tests, designed to understand the limits of patch-based attacks against SS.
% and compare against existing works.
The results of the experiments show that SS models tend to be reasonably robust to RWAEs, making them a strong candidate to consider for improving trustworthiness of the Deep Learning pipeline in safety-critical systems. To the best of our knowledge, this work represents the first exhaustive evaluation of the robustness of SS models against RWAEs for autonomous driving systems. 

%The achieved results clearly state how the tested SS models are often reasonably robust for a real-world environment and, therefore, RWAEs should be much more toward consideration for making trustworthy evaluations of Deep Learning in safety-critical systems.  To the best of our knowledge, this work represents the first exhaustive evaluation of the robustness of SS models against RWAEs for autonomous driving systems.


In summary, this paper makes the following novel contributions:
\begin{compactitem}
    \item it presents and evaluates a new state-of-the-art adversarial crafting pipeline for real-world adversarial patches, called scene-specific attack;
    \item it proposes an extension of the pixel-wise cross-entropy loss function, showing that it outperforms other formulations;
    \item it uses the CARLA simulator to perform inexpensive tests in realistic settings; and
    \item it reports some successful patch attacks in the real-world. As well also important statements on the robustness of SS models for a real-world attacks in Autonomous Driving Scenario. 
\end{compactitem}

% \begin{compactitem}
%     \item it presents and evaluates a new state-of-the-art adversarial crafting pipeline for real-world adversarial patches, called scene-specific attack, and compair it with an the EoT paradigm extended for SS patches for the first time;
%     \item it proposes an extension of the pixel-wise cross-entropy loss function. A comparison with original version applied by previous works is firstly presented for crafting digital adversarial patches. Then always applied to leverage the powerful of adversarial examples
%     \item it uses the CARLA simulator to perform inexpensive tests in realistic settings; and
%     \item it reports some successful real-world patch attacks. As well also important statements on the robustness of SS models for a real-world attacks in Autonomous Driving Scenario. 
% \end{compactitem}

The remainder of this paper is organized as follows: Section \ref{s:related} briefly reviews previous related work, Section \ref{s:method} presents the formulation of the contributions, Section \ref{s:exp} shows the experimental results, and Section \ref{s:conclusions} states the conclusions and proposes ideas for future work.

}
\end{comment}

\begin{comment}
 \color{blue} RWAEs are the focus of this paper as they represent a realistic threat to tasks in autonomous driving today. Though the effects of real-world adversarial examples have been studied extensively in the literature for classification and object detection, semantic segmentation remains relatively unexplored. Thus, this paper, among other things, examines the various start-of-the-art models for real-time semantic segmentation aiming to benchmark their robustness to RWAEs.

Of the several types of RWAEs proposed in the literature \cite{sun_survey_2018}, the form of attack used in this paper is Adversarial Patches \cite{brown_adversarial_2018}. Such patches can be easily printed and attached to any visible 2D surface in the driving environment, such as billboards and road signs, thus making them a simple, yet effective attack strategy.

The paper starts by recognizing the shortcomings of the standard cross-entropy loss for optimizing adversarial patches for SS. Thus, an extension to the cross-entropy loss is proposed. This extension forces the optimization to focus on pixels that are not yet misclassified. The patches thus crafted are more powerful compared to those generated with the standard cross-entropy-based setting.

Following this, the robustness of real-time SS models to RWAE attacks was benchmarked. These experiments were performed on the Cityscapes dataset \cite{DBLP:conf/cvpr/CordtsORREBFRS16}, a popular benchmark for tasks in urban driving. Since Expectation Over Transformation (EOT) \cite{pmlr-v80-athalye18b} is the accepted paradigm for real-world attacks, the study compares patches optimized with and without EOT. Thus, for this, an extension to EOT for the case of semantic segmentation is presented. As a result of these experiments, a set of transformations fit for EOT optimizations for autonomous driving scenarios are presented. 

Despite the benefits of the EOT-based approach, evaluating these patches within the CARLA simulator \cite{2017arXiv171103938D} did not always produce satisfactory results. The EOT-based approach appeared to work well when the attacked surface, in this case, a billboard, was perpendicular to the road and hence in clear view of the camera. But for billboards at an angle to the road, the perturbations were concentrated within the proximity of the patch. Thus, a new approach to crafting adversarial patches, named  \emph{scene-specific attack}, is proposed. This new technique is more realistic as it assumes that the attacker is interested in targeting a particular area of the town, allowing the attacker to craft new patches with a smaller set of examples while also exploiting geometric information about the billboard. The proposed approach allows for more accurate projections of the patch during training, thereby leading to crafting more effective patches, even with billboards placed at an angle to the road.

All experiments in the paper were performed using a unified pipeline. The said pipeline allowed the flexibility of seamlessly shifting between different datasets and different attack strategies. This pipeline was further tested by crafting an EOT-based patch for a selected locality within our town. The patch thus generated was printed to evaluate the effectiveness of the patch in the physical world.

In summary, the paper makes the following contributions:
\begin{compactitem}
 \item It proposes an extension to the pixel-wise cross-entropy loss to enable crafting strong patches for the semantic segmentation setting
 \item It reports a benchmark of RWAE attacks on a set of real-time semantic segmentation models using the Cityscapes dataset
 \item It proposes a novel technique for crafting adversarial patches for autonomous driving scenarios that utilize geometric information of the 3D world
 \item It presents a pipeline that enables quick, flexible and seamless crafting and evaluation of adversarial patches on a range of datasets from Cityscapes to the simulator and even to the physical world. 
\end{compactitem}

The remainder of this paper is organized as follows: Section \ref{s:related} provides a brief overview of related work existing in the literature, Section \ref{s:method} formalizes the proposed loss function, pipeline and attack strategy, Section \ref{s:exp} reports the experimental results, and Section \ref{s:conclusions} states the conclusions and proposes ideas for future work.

\end{comment}


==> arxiv - Copia/related.tex <==
\section{Related Work} \label{s:related}

%This section highlights the differences between digital and physical adversarial attacks. It then goes on to explain how physical attacks can be crafted using the EOT algorithm.

%\subsection{Adversarial Attacks}
Szegedy et al. \cite{DBLP:journals/corr/SzegedyZSBEGF13} showed that small well-crafted perturbations when added to the input image were sufficient to fool strong classification networks. %This has established the field of ‘adversarial machine learning’ to study why neural networks are prone to such attacks, how these attacks can be crafted and how one can defend against them. 
%Other works \cite{DBLP:conf/sp/Carlini017, DBLP:conf/cvpr/Moosavi-Dezfooli16, 2016arXiv161008401M} have introduced more efficient techniques for crafting adversarial attacks. 
\cite{bar_vulnerability_2021, 
metzen_universal_2017, 
DBLP:conf/iccv/XieWZZXY17,  
DBLP:journals/access/KangSDG20, 
2019arXiv190805005K,  
arnab_robustness_nodate, 
nakka_indirect_2019,
shen2019advspade} have studied such attacks for the specific use case of fooling SS models. However, these attacks directly manipulate the pixels of the image. Although such digital perturbations provide a convenient way to provide benchmarks in research, they do no extend well to real-world applications.
%However, these attacks do not present a realistic threat model for an autonomous driving scenario. The work in these papers build on the assumption that the attacker has access to the digital representation of the image before it is fed to the network, such that the attacker can inject noise into the input (\emph{digital} adversarial attacks).

%input. Such techniques fall under the category of \emph{digital adversarial attacks}. 

A more realistic threat model led to the introduction of RWAEs by Kurakin et. al. \cite{kurakin_adversarial_2017}. The attacker here is assumed to be able to craft adversarial pictures in the physical world, without the ability to manipulate the digital representation of inputs to the neural network. However, this work did not account for factors that affect images of objects in the real-world (e.g., varying viewpoints from which input images could be captured, changes in lighting conditions and so on). Athalye et. al. \cite{pmlr-v80-athalye18b} address this issue by introducing the EOT algorithm. EOT accounts for such factors in the optimisation by modeling them as a distribution of transformation functions applied to the adversarial input. These transformations can be in the form of rotation, scaling, noise, brightening and so on. Then, the idea is to optimize the loss function in expectation across the range of selected transformation functions.

%{\color{blue} 
%Although the latter approaches are closer to a real-world robustness evaluation, crafting adversarial object is notably more challenging and costly than digital perturbation, especially due to the need of a 3D testing environments. 
%X et al 1, Y et al 2 realized adversarial objects based on the EOT paradigm and capable to fool a DNN lidar system in 3D environments, while, to the best of our knowledge not works provide real world evaluation for an image based system processed with a SS model. 
%For image based system instead an objected always interpreted as its 2D projection that appears as a patch on the received image. 
The EOT formulation led to the development of \emph{adversarial patches}, introduced by Brown et al.~\cite{brown_adversarial_2018} to fool image classifiers. They are robust, localized, image-agnostic perturbations, crafted with the EOT paradigm, capable of fooling neural networks when placed within the input scene or added digitally on images. 

Although extensive prior work exists to construct such physical attacks for classification~\cite{brown_adversarial_2018, sharif_accessorize_2016, eykholt_robust_2018}, object detection \cite{DBLP:conf/eccv/WuLDG20, wu_physical_2020, lee_physical_2019, zhang_camou_2019}, optical flow \cite{2019arXiv191010053R}, LiDAR object detection \cite{Tu2020PhysicallyRA}, and depth estimation \cite{2020arXiv201003072Y}, only a few focus on autonomous driving tasks, since testing the adversarial robustness is more challenging, as it requires controlling the 3D outdoor environments. %To face the latter issue, famous car simulators help enormously in managing virtual testing scenarios for crafting adversarial situations. As such, also some of the previous works (e.g., [CITE WORKS THAT USE CARLA]) exploit those frameworks for accomplishing their attacks. Similarly, this work involves Carla [CITE] in part of our tests, as one of the most famous and complete simulation tools.
Other works \cite{zhang_camou_2019, wu_physical_2020} have shown CARLA to be a viable solution in alleviating this issue by crafting and evaluating adversarial situations in virtual 3D environments. This paper also heavily relies on CARLA to evaluate how the optimized adversarial patches translate to a 3D world.

%Concluding the discussion on studies addressed at investigating the robustness of autonomous driving components, X of Lidar X, depth estimator X and object detection X. However, 

The work closest to ours is the one by Nakka et. al. \cite{nakka_indirect_2019}, who attempted to fool a variety of SS models via local attacks (i.e., creating pixel perturbation in a specific area of the image). Despite the attacks being local, the objective of their study was not to evaluate the robustness to real-world attacks, which is instead the main focus of this paper.
%However, despite being local, unlike our work, the objective of their attacks doesn't pose particular efforts on the real-world robustness.
To the best of our knowledge, such a study is missing in the literature for the case of SS models, which represent essential components in an autonomous driving perception pipeline \cite{siam2018comparative}. 
%The attack scheme provided in this paper include not negligible transformations in the optimization process to produce powerful patches for SS models in autunomous driving scenario that can be placed inside the tested dataset in order to extract a more realistic assessment.

%In this particular scenario, additional real-world constraints for reinforcing the robustness of adversarial objects are needed to enhance to their robustness even against brightness ADD... [CITE SOMEONE]. . LIST addressed to the outdoor autonomous car environment. CITE all the works
%In this domain, additional challenging arise to studying adversarial weaknesses of the model. The first one is about the need of testing a real 3D outdoor environment.
%Second, when 
%to the best of our knowledge, such a study does not exist for SS model, which is one of the most important component of an autonomous driving perception pipeline [CITE]. 

%Finally, it is worth to mention more theoretically works, such as X, that present an insight analysis of the real-world robustness for DNN models, however more practical evaluations are needed to clarify the real effectiveness of real-world attacks.

Additionally, this paper also improves the loss function used for generating patches. 
Section \ref{subsection:loss} presents a more general formulation of the cross-entropy loss for the SS setting, designed to optimize more powerful and effective adversarial examples, while all the previously mentioned papers use the standard pixel-wise cross-entropy loss. 

%Finally, as far as concerned the proposed SS attack scheme, important considerations should be devoted to the loss function used to guide the adversarial optimization process. The above-mentioned adversarial works addressed on SS models employ the common pixel-wise cross-entropy loss function, while, in Section \ref{fig:attack_scheme}, a novel loss function formulation is illustrated to improve the adversarial optimization achieving more effective digital and real-world patches.

%\subsection{Expectation Over Transformation}
%Approaches that work well in digital adversarial attacks, often fail when moved to the physical realm \cite{DBLP:journals/corr/LuSFF17}. This failure can be attributed to changes in viewing angles, differences in lighting conditions, and other factors beyond the control of the attacker. 
%}
